PDT: Pretrained Dual Transformers for Time-aware Bipartite Graphs

Pre-training on large models is prevalent and emerging with the ever-growing user-generated content in many machine learning application categories. It has been recognized that learning contextual knowledge from the datasets depicting user-content interaction plays a vital role in downstream tasks. Despite several studies attempting to learn contextual knowledge via pre-training methods, finding an optimal training objective and strategy for this type of task remains a challenging problem. In this work, we contend that there are two distinct aspects of contextual knowledge, namely the user-side and the content-side, for datasets where user-content interaction can be represented as a bipartite graph. To learn contextual knowledge, we propose a pre-training method that learns a bi-directional mapping between the spaces of the user-side and the content-side. We formulate the training goal as a contrastive learning task and propose a dual-Transformer architecture to encode the contextual knowledge. We evaluate the proposed method for the recommendation task. The empirical studies have demonstrated that the proposed method outperformed all the baselines with significant gains.

==> tab_case_study_embedding_old.tex <==
 \begin{table*}[!ht]
     %\label{tab:case_study2}
     \centering
     \caption{10 nearest neighbors of "Avengers: Infinity War - Part I"}
     \begin{tabular}{ll}
     \toprule
     Title    & Genre \\ 
     \midrule
     Kingsman: The Secret Service & Action|Adventure|Comedy|Crime \\
     Avengers: Infinity War - Part II &	Action|Adventure|Sci-Fi \\
     Thor: Ragnarok & Action|Adventure|Sci-Fi \\
     Guardians of the Galaxy 2 & Action|Adventure|Sci-Fi \\
     Zootopia & Action|Adventure|Animation|Children|Comedy \\
     Rogue One: A Star Wars Story & Action|Adventure|Fantasy|Sci-Fi \\
     Logan &	Action|Sci-Fi \\
     Coco & Adventure|Animation|Children \\
     Deadpool 2 & Action|Comedy|Sci-Fi \\
     Spider-Man: Into the Spider-Verse &	Action|Adventure|Animation|Sci-Fi \\
     
     \bottomrule
     \end{tabular}
     \label{tab:case_study2}
 \end{table*}
  
 \begin{table*}[!ht]
     %\label{tab:case_study1}
     \centering
     \caption{10 nearest neighbors of "Harry Potter and the Sorcerer's Stone"}
     \begin{tabular}{ll}
     \toprule
     Title    & Genre \\ 
     \midrule
     Harry Potter and the Chamber of Secrets  & Adventure|Fantasy \\
     Harry Potter and the Prisoner of Azkaban &	Adventure|Fantasy|IMAX \\
     Spider-Man  &  Action|Adventure|Sci-Fi|Thriller \\
     Spider-Man 2 &	Action|Adventure|Sci-Fi|IMAX\\
     Star Wars: Episode II - Attack of the Clones  &	Action|Adventure|Sci-Fi|IMAX \\
     Star Wars: Episode III - Revenge of the Sith &	Action|Adventure|Sci-Fi\\
     X2: X-Men United  & Action|Adventure|Sci-Fi|Thriller \\
     Matrix Reloaded  &	Action|Adventure|Sci-Fi|Thriller|IMAX \\
     Shrek 2  &	Adventure|Animation|Children|Comedy|Musical|Romance \\
     Bourne Supremacy & Action|Crime|Thriller \\
     
     \bottomrule
     \end{tabular}
     \label{tab:case_study1}
  \end{table*}

  \begin{table*}[!ht]
     %\label{tab:case_study3}
     \centering
     \caption{10 nearest neighbors of "The Babysitter"}
     \begin{tabular}{ll}
     \toprule
     Title    & Genre \\ 
     \midrule
     Oculus & Horror \\
     The Voices & Comedy|Crime|Thriller \\
     Unfriended & Horror|Mystery|Thriller \\
     The Visit & Comedy|Horror \\
     Circle & Drama|Horror|Sci-Fi \\
     The Boy & Horror|Thriller\\
     Hush & Thriller \\
     The Shallows & Drama|Thriller \\
     Lights Out & Horror \\
     The Autopsy of Jane Doe & Horror \\ 
     \bottomrule
     \end{tabular}
     \label{tab:case_study3}
  \end{table*}





==> tab_results_movielens_acm.tex <==


 \begin{table*}[!ht]
     % \scriptsize
     \label{tab:comparison}
     \centering
     \begin{tabular}{c|ccccc|cccc|cc}
     \toprule
     \multirow{2}{*}{Metric} & \multicolumn{5}{c|}{General Recommender} & \multicolumn{4}{c|}{Sequential Recommender} &   \multicolumn{2}{c}{Ours}       \\ \cline{2-12}
                             & BPR-MF  & NeuMF & NGCF & LightGCN & SGL & GRU4Rec   & SASRec   & BERT4Rec  & S3-Rec  & PDT & Improv. \\
                             \midrule
     Recall@10               &         &       &      &          &     &           &          &           &         &      &         \\
     Recall@20               &         &       &      &          &     &           &          &           &         &      &         \\
     Recall@50               &         &       &      &          &     &           &          &           &         &      &         \\
     NDCG@10                 &         &       &      &          &     &           &          &           &         &      &         \\
     NDCG@20                 &         &       &      &          &     &           &          &           &         &      &         \\
     NDCG@50                 &         &       &      &          &     &           &          &           &         &      &         \\
     \bottomrule
     \end{tabular}
 \end{table*}



==> tab_results_movielens_acm2.tex <==
 \begin{table*}[!ht]
     \label{tab:comparison}
     \centering
     \begin{tabular}{ccccccccccc}
     \toprule
     Metric    & BPR-MF & NeuMF & NGCF & LightGCN & SGL & GRU4Rec & SASRec & BERT4Rec & Ours & Improv. \\ 
     \midrule
     Recall@10 &        &       &      &          &     &         &        &          &      &         \\
     Recall@20 &        &       &      &          &     &         &        &          &      &         \\
     Recall@50 &        &       &      &          &     &         &        &          &      &         \\
     NDCG@10   &        &       &      &          &     &         &        &          &      &         \\
     NDCG@20   &        &       &      &          &     &         &        &          &      &         \\
     NDCG@50   &        &       &      &          &     &         &        &          &      &         \\ 
     \bottomrule
     \end{tabular}
 \end{table*}
